Achievable Rates for Short-Reach Fiber-Optic Channels with Direct Detection

Spectrally efficient communication is studied for short-reach fiber-optic links with chromatic dispersion (CD) and receivers that employ direction-detection and oversampling. Achievable rates and symbol error probabilities are computed by using auxiliary channels that account for memory in the sampled symbol strings. Real-alphabet bipolar and complex-alphabet symmetric modulations are shown to achieve significant energy gains over classic intensity modulation. Moreover, frequency-domain raised-cosine (FD-RC) pulses outperform time-domain RC (TD-RC) pulses in terms of spectral efficiency for two scenarios. First, if one shares the spectrum with other users then inter-channel interference significantly reduces the TD-RC rates. Second, if there is a transmit filter to avoid interference then the detection complexity of FD-RC and TD-RC pulses is similar but FD-RC achieves higher rates.

==> Figures/standalone/Q2/dataQ2_MI_TXPOW.tex <==
\pgfplotstableread{
    X Y
-2	0.0394838650590552
-1	0.0604822781111869
0	0.092910423846563
1	0.143802682408492
2	0.223244652495882
3	0.318059829271708
4	0.441491524925217
5	0.58305071896579
6	0.738735525023364
7	0.862889273024182
8	0.939244861848263
9	0.983752349656461
10	0.997850028113214
11	0.999759896468802
12	1.00003617817338
13	0.999972530856557
14	1.00005999877349
15	0.999937869314056
16	1.00004554036649
17	1.00005245727031
18	1.00005994130074
19	-1
20	-1
}{\PAMrcosspanthree}


\pgfplotstableread{
    X Y
-2	0.0405212455927835
-1	0.0624179837395697
0	0.0961794260857136
1	0.147972562871276
2	0.229998862556564
3	0.325155600718338
4	0.452814020595225
5	0.599647133431676
6	0.752120123481131
7	0.876957100381308
8	0.948607201375963
9	0.986840742540818
10	0.998069753905512
11	0.999956375198743
12	1.00005498476621
13	1.00008372949827
14	0.999924499558243
15	1.00009722309147
16	1.000092991293
17	0.999938497140931
18	1.00009983357399
19	0.999381514315012
20	0.99855299019346
}{\PAMrcosspanfive}


\pgfplotstableread{
    X Y
-13.0000    0.0039
  -12.0000    0.0060
  -11.0000    0.0092
  -10.0000    0.0155
   -9.0000    0.0272
   -8.0000    0.0400
   -7.0000    0.0606
   -6.0000    0.0898
   -5.0000    0.1460
   -4.0000    0.2168
   -3.0000    0.3095
   -2.0000    0.4363
   -1.0000    0.5843
         0    0.7305
    1.0000    0.8609
    2.0000    0.9427
    3.0000    0.9822
    4.0000    0.9971
    5.0000    0.9998
    6.0000    0.9999
    7.0000    1.0000
    8.0000    1.0001
    9.0000    1.0001
   10.0000    1.0000
   11.0000    1.0001
   12.0000    1.0001
   13.0000    1.0000
   14.0000    1.0000
   15.0000    1.0000
   16.0000    1.0000
   17.0000    0.9999
   18.0000    1.0000
}{\PAMrcosspanseven}


\pgfplotstableread{
    X Y
-13.0000    0.0040
  -12.0000    0.0061
  -11.0000    0.0093
  -10.0000    0.0156
   -9.0000    0.0278
   -8.0000    0.0404
   -7.0000    0.0614
   -6.0000    0.0906
   -5.0000    0.1474
   -4.0000    0.2188
   -3.0000    0.3123
   -2.0000    0.4401
   -1.0000    0.5893
         0    0.7358
    1.0000    0.8653
    2.0000    0.9459
    3.0000    0.9842
    4.0000    0.9972
    5.0000    0.9997
    6.0000    1.0000
    7.0000    1.0000
    8.0000    1.0000
    9.0000    1.0001
   10.0000    1.0000
   11.0000    1.0000
   12.0000    1.0000
   13.0000    1.0000
   14.0000    1.0000
   15.0000    1.0001
   16.0000    0.9999
   17.0000    0.9997
   18.0000    1.0000
}{\PAMrcosspannine}


\pgfplotstableread{
    X Y
 -13.0000    0.0040
  -12.0000    0.0061
  -11.0000    0.0093
  -10.0000    0.0158
   -9.0000    0.0278
   -8.0000    0.0407
   -7.0000    0.0618
   -6.0000    0.0915
   -5.0000    0.1481
   -4.0000    0.2198
   -3.0000    0.3148
   -2.0000    0.4431
   -1.0000    0.5925
         0    0.7413
    1.0000    0.8711
    2.0000    0.9501
    3.0000    0.9853
    4.0000    0.9974
    5.0000    0.9997
    6.0000    1.0001
    7.0000    1.0000
    8.0000    1.0000
    9.0000    1.0001
   10.0000    1.0001
   11.0000    1.0000
   12.0000    1.0000
   13.0000    1.0001
   14.0000    1.0001
   15.0000    1.0001
   16.0000    0.9999
   17.0000    1.0000
   18.0000    1.0000
}{\PAMrcosspaneleven}



\pgfplotstableread{
    X Y
-2	0.0173512348293725
-1	0.026904431207865
0	0.0430096589857882
1	0.065874246301072
2	0.098372277797691
3	0.14501266724076
4	0.212578363530939
5	0.29020221863479
6	0.378370067682124
7	0.473578037685493
8	0.546268916965663
9	0.58176856711662
10	0.558767867949388
11	0.468068713386876
12	0.330280899538802
13	0.0834079067002156
14	-0.296945749969753
15	-1.06546880829734
16	-1.97788460455382
17	-3.61273812146406
18	-6.44761303643796
19	-1
20	-1
}{\ASKrcosspanthree}


\pgfplotstableread{
    X Y
-2	0.0188953861389978
-1	0.0298744677251177
0	0.0467502720255268
1	0.0717789402305344
2	0.10789608189399
3	0.160126443904224
4	0.235131562588412
5	0.324749089254124
6	0.429606090095781
7	0.542487456252683
8	0.639083275469287
9	0.71655102178061
10	0.764473602822478
11	0.775824811497979
12	0.768580232784624
13	0.718751029070927
14	0.64367289144505
15	0.446361389976688
16	0.261481389266208
17	-0.126668630177033
18	-0.859433844204027
19	-1.90940902144448
20	-3.34909494553779
}{\ASKrcosspanfive}


\pgfplotstableread{
    X Y
-13.0000    0.0024
  -12.0000    0.0030
  -11.0000    0.0053
  -10.0000    0.0072
   -9.0000    0.0132
   -8.0000    0.0220
   -7.0000    0.0308
   -6.0000    0.0485
   -5.0000    0.0756
   -4.0000    0.1119
   -3.0000    0.1650
   -2.0000    0.2302
   -1.0000    0.3186
         0    0.4050
    1.0000    0.4884
    2.0000    0.5638
    3.0000    0.6158
    4.0000    0.6593
    5.0000    0.6567
    6.0000    0.6661
    7.0000    0.6753
    8.0000    0.6773
    9.0000    0.6729
   10.0000    0.6786
   11.0000    0.6604
   12.0000    0.6547
   13.0000    0.6566
   14.0000    0.6804
   15.0000    0.6727
   16.0000    0.6625
   17.0000    0.6874
   18.0000    0.6634
}{\ASKrcosspanseven}


\pgfplotstableread{
    X Y
 -13.0000    0.0024
  -12.0000    0.0033
  -11.0000    0.0055
  -10.0000    0.0074
   -9.0000    0.0135
   -8.0000    0.0229
   -7.0000    0.0320
   -6.0000    0.0504
   -5.0000    0.0787
   -4.0000    0.1163
   -3.0000    0.1702
   -2.0000    0.2393
   -1.0000    0.3334
         0    0.4238
    1.0000    0.5139
    2.0000    0.5973
    3.0000    0.6519
    4.0000    0.6980
    5.0000    0.6970
    6.0000    0.7038
    7.0000    0.7152
    8.0000    0.7152
    9.0000    0.7052
   10.0000    0.7115
   11.0000    0.6912
   12.0000    0.6894
   13.0000    0.6894
   14.0000    0.7152
   15.0000    0.7004
   16.0000    0.6886
   17.0000    0.7179
   18.0000    0.6949
}{\ASKrcosspannine}


\pgfplotstableread{
    X Y
 -13.0000    0.0025
  -12.0000    0.0034
  -11.0000    0.0057
  -10.0000    0.0076
   -9.0000    0.0139
   -8.0000    0.0233
   -7.0000    0.0330
   -6.0000    0.0518
   -5.0000    0.0806
   -4.0000    0.1191
   -3.0000    0.1747
   -2.0000    0.2473
   -1.0000    0.3419
         0    0.4373
    1.0000    0.5358
    2.0000    0.6207
    3.0000    0.6800
    4.0000    0.7328
    5.0000    0.7312
    6.0000    0.7385
    7.0000    0.7564
    8.0000    0.7509
    9.0000    0.7413
   10.0000    0.7524
   11.0000    0.7253
   12.0000    0.7228
   13.0000    0.7146
   14.0000    0.7486
   15.0000    0.7354
   16.0000    0.7270
   17.0000    0.7535
   18.0000    0.7293
}{\ASKrcosspaneleven}

\pgfplotstableread{
X Y
  -13.0000    0.0025
  -12.0000    0.0036
  -11.0000    0.0057
  -10.0000    0.0075
   -9.0000    0.0141
   -8.0000    0.0237
   -7.0000    0.0337
   -6.0000    0.0530
   -5.0000    0.0819
   -4.0000    0.1213
   -3.0000    0.1776
   -2.0000    0.2523
   -1.0000    0.3500
         0    0.4478
    1.0000    0.5519
    2.0000    0.6399
    3.0000    0.7038
    4.0000    0.7600
    5.0000    0.7639
    6.0000    0.7712
    7.0000    0.7826
    8.0000    0.7806
    9.0000    0.7748
   10.0000    0.7821
   11.0000    0.7557
   12.0000    0.7545
   13.0000    0.7436
   14.0000    0.7834
   15.0000    0.7625
   16.0000    0.7545
   17.0000    0.7780
   18.0000    0.7524
}{\ASKrcosspanthirten}

\pgfplotstableread{
X Y
  -13.0000    0.0026
  -12.0000    0.0036
  -11.0000    0.0058
  -10.0000    0.0075
   -9.0000    0.0142
   -8.0000    0.0238
   -7.0000    0.0341
   -6.0000    0.0533
   -5.0000    0.0829
   -4.0000    0.1224
   -3.0000    0.1804
   -2.0000    0.2567
   -1.0000    0.3558
         0    0.4578
    1.0000    0.5627
    2.0000    0.6562
    3.0000    0.7214
    4.0000    0.7817
    5.0000    0.7861
    6.0000    0.7978
    7.0000    0.8118
    8.0000    0.8117
    9.0000    0.8035
   10.0000    0.8053
   11.0000    0.7844
   12.0000    0.7751
   13.0000    0.7704
   14.0000    0.8078
   15.0000    0.7839
   16.0000    0.7788
   17.0000    0.8003
   18.0000    0.7837
}{\ASKrcosspanfiften}

\pgfplotstableread{
    X Y
      -13.0000    0.0026
  -12.0000    0.0037
  -11.0000    0.0059
  -10.0000    0.0076
   -9.0000    0.0142
   -8.0000    0.0240
   -7.0000    0.0344
   -6.0000    0.0538
   -5.0000    0.0835
   -4.0000    0.1239
   -3.0000    0.1823
   -2.0000    0.2597
   -1.0000    0.3596
         0    0.4648
    1.0000    0.5731
    2.0000    0.6690
    3.0000    0.7366
    4.0000    0.7985
    5.0000    0.8079
    6.0000    0.8205
    7.0000    0.8343
    8.0000    0.8375
    9.0000    0.8290
   10.0000    0.8327
   11.0000    0.8164
   12.0000    0.8075
   13.0000    0.8013
   14.0000    0.8314
   15.0000    0.8041
   16.0000    0.8038
   17.0000    0.8259
   18.0000    0.8145
   }{\ASKrcosspanseventen}






\pgfplotstableread{
    X Y
-13.0000    0.0042
  -12.0000    0.0066
  -11.0000    0.0104
  -10.0000    0.0165
   -9.0000    0.0259
   -8.0000    0.0407
   -7.0000    0.0636
   -6.0000    0.0985
   -5.0000    0.1509
   -4.0000    0.2276
   -3.0000    0.3361
   -2.0000    0.4838
   -1.0000    0.6764
         0    0.9170
    1.0000    1.2065
    2.0000    1.5444
    3.0000    1.9298
    4.0000    2.3613
    5.0000       Inf
    6.0000       Inf
    7.0000       Inf
    8.0000       Inf
    9.0000       Inf
   10.0000       Inf
   11.0000       Inf
   12.0000       Inf
   13.0000       Inf
   14.0000       Inf
   15.0000       Inf
   16.0000       Inf
   17.0000       Inf
   18.0000       Inf
}{\PAMCovUpperBound}


\pgfplotstableread{
    X Y
  -13.0000    0.0024
  -12.0000    0.0037
  -11.0000    0.0059
  -10.0000    0.0094
   -9.0000    0.0148
   -8.0000    0.0232
   -7.0000    0.0364
   -6.0000    0.0567
   -5.0000    0.0875
   -4.0000    0.1331
   -3.0000    0.1991
   -2.0000    0.2908
   -1.0000    0.4131
         0    0.5688
    1.0000    0.7578
    2.0000    0.9778
    3.0000    1.2246
    4.0000    1.4934
    5.0000    1.7795
    6.0000    2.0789
    7.0000    2.3882
    8.0000       Inf
    9.0000       Inf
   10.0000       Inf
   11.0000       Inf
   12.0000       Inf
   13.0000       Inf
   14.0000       Inf
   15.0000       Inf
   16.0000       Inf
   17.0000       Inf
   18.0000       Inf
   }{\ASKCovUpperBound}




==> Figures/standalone/Q2/dataQ2_SER_TXPOW.tex <==



\pgfplotstableread{
    X Y
  -13.0000    0.4743
  -12.0000    0.4643
  -11.0000    0.4581
  -10.0000    0.4464
   -9.0000    0.4273
   -8.0000    0.4101
   -7.0000    0.3896
   -6.0000    0.3654
   -5.0000    0.3255
   -4.0000    0.2839
   -3.0000    0.2387
   -2.0000    0.1854
   -1.0000    0.1302
         0    0.0800
    1.0000    0.0385
    2.0000    0.0134
    3.0000    0.0044
    4.0000    0.0008
    5.0000    0.0002
    6.0000    0.0001
    7.0000    0.0001
    8.0000    0.0002
    9.0000    0.0001
   10.0000    0.0001
   11.0000    0.0001
   12.0000    0.0001
   13.0000    0.0002
   14.0000    0.0002
   15.0000    0.0001
   16.0000    0.0001
   17.0000    0.0002
   18.0000    0.0001

}{\PAMrcosspanseventeen}




\pgfplotstableread{
    X Y
  -13.0000    0.4845
  -12.0000    0.4790
  -11.0000    0.4713
  -10.0000    0.4659
   -9.0000    0.4534
   -8.0000    0.4409
   -7.0000    0.4306
   -6.0000    0.4093
   -5.0000    0.3860
   -4.0000    0.3612
   -3.0000    0.3284
   -2.0000    0.2933
   -1.0000    0.2501
         0    0.2056
    1.0000    0.1643
    2.0000    0.1200
    3.0000    0.0853
    4.0000    0.0568
    5.0000    0.0451
    6.0000    0.0384
    7.0000    0.0304
    8.0000    0.0270
    9.0000    0.0269
   10.0000    0.0245
   11.0000    0.0255
   12.0000    0.0264
   13.0000    0.0257
   14.0000    0.0236
   15.0000    0.0243
   16.0000    0.0244
   17.0000    0.0223
   18.0000    0.0234
   }{\ASKrcosspanseventeen}


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

